Contracting the Facebook API

In recent years, there has been an explosive growth in the popularity of online social networks such as Facebook. In a new twist, third party developers are now able to create their own web applications which plug into Facebook and work with Facebook's "social" data, enabling the entire Facebook user base of more than 400 million active users to use such applications. These client applications can contain subtle errors that can be hard to debug if they misuse the Facebook API. In this paper we present an experience report on applying Microsoft's new code contract system for the .NET framework to the Facebook API.We wrote contracts for several classes in the Facebook API wrapper which allows Microsoft .NET developers to implement Facebook applications. We evaluated the usefulness of these contracts during implementation of a new Facebook application. Our experience indicates that having code contracts provides a better and quicker software development experience.

==> eptcsdata.tex <==
\providecommand{\firstpage}{63}
\providecommand{\publicationstatus}{Sala\"un, Fu, and Hall\'e (Eds.): Fourth International Workshop\\
on Testing, Analysis and Verification of Web Software\\
EPTCS 35, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.35.6}{10.4204/EPTCS.35.6}}

